Enhancing the signal-to-noise ratio of solar-like targets

The analysis of the first solar-like targets done by CoRoT has shown that the oscillation amplitudes are about 25% below the theoretical amplitudes while the convective backgrounds are up to three times higher than in the solar case (Michel et al. 2008). In such conditions, the comb-like structure of the acoustic modes has smaller signal-to-noise ratios than initially expected complicating the characterization of individual modes. In the present work we apply the curvelet filtering to the solar-like targets already observed by CoRoT as well as a partial reconstruction of the signal from the obtained spacing of the comb-like structure of the acoustic modes. It enables us to enhance the signal-to-noise ratio of the ridges in the Echelle diagrams. Finally, we study how the analysis of the p modes can be improved.

==> PaxHeader/Garcia_enhance_v1.tex <==
18 gid=2048330233
17 uid=174949570
20 ctime=1269436677
20 atime=1269436681
38 LIBARCHIVE.creationtime=1269294814
24 SCHILY.dev=234881026
22 SCHILY.ino=1721206
18 SCHILY.nlink=1

